raceBERT -- A Transformer-based Model for Predicting Race and Ethnicity from Names

This paper presents raceBERT -- a transformer-based model for predicting race and ethnicity from character sequences in names, and an accompanying python package. Using a transformer-based model trained on a U.S. Florida voter registration dataset, the model predicts the likelihood of a name belonging to 5 U.S. census race categories (White, Black, Hispanic, Asian & Pacific Islander, American Indian & Alaskan Native). I build on Sood and Laohaprapanon (2018) by replacing their LSTM model with transformer-based models (pre-trained BERT model, and a roBERTa model trained from scratch), and compare the results. To the best of my knowledge, raceBERT achieves state-of-the-art results in race prediction using names, with an average f1-score of 0.86 -- a 4.1% improvement over the previous state-of-the-art, and improvements between 15-17% for non-white names.

==> tables/ethncity_performance_scratch.tex <==
\begin{tabular}{lrrrrr}
\toprule
metric &  precision &  recall &    f1 &  ethnicolr\_f1 &  \% improvement \\
group                                 &            &         &       &               &                \\
\midrule
Asian,GreaterEastAsian,EastAsian      &       0.76 &    0.79 &  0.77 &          0.82 &          -5.81 \\
Asian,GreaterEastAsian,Japanese       &       0.88 &    0.84 &  0.86 &          0.90 &          -4.38 \\
Asian,IndianSubContinent              &       0.73 &    0.74 &  0.73 &          0.77 &          -4.99 \\
GreaterAfrican,Africans               &       0.45 &    0.40 &  0.42 &          0.49 &         -15.40 \\
GreaterAfrican,Muslim                 &       0.59 &    0.72 &  0.65 &          0.67 &          -3.34 \\
GreaterEuropean,British               &       0.80 &    0.82 &  0.81 &          0.82 &          -1.29 \\
GreaterEuropean,EastEuropean          &       0.74 &    0.73 &  0.74 &          0.76 &          -3.21 \\
GreaterEuropean,Jewish                &       0.48 &    0.51 &  0.49 &          0.47 &           4.68 \\
GreaterEuropean,WestEuropean,French   &       0.71 &    0.61 &  0.66 &          0.64 &           2.66 \\
GreaterEuropean,WestEuropean,Germanic &       0.54 &    0.40 &  0.46 &          0.46 &           0.09 \\
GreaterEuropean,WestEuropean,Hispanic &       0.73 &    0.65 &  0.69 &          0.70 &          -1.86 \\
GreaterEuropean,WestEuropean,Italian  &       0.70 &    0.75 &  0.73 &          0.75 &          -3.39 \\
GreaterEuropean,WestEuropean,Nordic   &       0.63 &    0.69 &  0.66 &          0.68 &          -3.37 \\
avg                                   &       0.71 &    0.71 &  0.71 &          0.73 &          -2.54 \\
\bottomrule
\end{tabular}

